An adaptive virtual element method for the polymer self-consistent field theory

In this paper, we develop a high-order adaptive virtual element method (VEM) to simulate the self-consistent field theory (SCFT) model in arbitrary domains. The VEM is very flexible in handling general polygon elements and can treat hanging nodes as polygon vertices without additional processing. Besides, to effectively simulate the phase separation behavior in strong segregation systems, an adaptive method on polygonal mesh equipped with a new marking strategy is developed. This new marking strategy will indicate the times of marked elements to be refined and coarsened, making full use of the information contained in the current numerical results. Using the halfedge data structure, we can apply the adaptive method to the arbitrary polygonal mesh. Numerical results demonstrate that the developed method is efficient in simulating polymers' phase behavior in complex geometric domains. The accuracy is consistent with theoretical results. The adaptive method can greatly reduce computational costs to obtain prescribed numerical accuracy for strong segregation systems.

==> backup.tex <==

In this paper, we develop a high-order adaptive virtual element method (VEM) to
simulate the self-consistent field theory (SCFT) model in arbitrary domains.
The VEM is very flexible in handling general polygon elements, which can treat
hanging points as polygon vertexes without additional processing.  It is more
suitable to discrete the model defined on complex geometric domains. In
addition, to effectively simulate the phase separation behavior in strong
segregation systems, an adaptive method on polygonal mesh equipped with a new
marking strategy is developed. This new marking strategy will indicate the times 
of marked elements which should be refined and coarsened which can make full use of
the information contained in the current numerical results. The numerical tests
show that the proposed adaptive method can obtain ideal accuracy with less
computational cost.


